Learning Interacting Dynamical Systems with Latent Gaussian Process ODEs

We study time uncertainty-aware modeling of continuous-time dynamics of interacting objects. We introduce a new model that decomposes independent dynamics of single objects accurately from their interactions. By employing latent Gaussian process ordinary differential equations, our model infers both independent dynamics and their interactions with reliable uncertainty estimates. In our formulation, each object is represented as a graph node and interactions are modeled by accumulating the messages coming from neighboring objects. We show that efficient inference of such a complex network of variables is possible with modern variational sparse Gaussian process inference techniques. We empirically demonstrate that our model improves the reliability of long-term predictions over neural network based alternatives and it successfully handles missing dynamic or static information. Furthermore, we observe that only our model can successfully encapsulate independent dynamics and interaction information in distinct functions and show the benefit from this disentanglement in extrapolation scenarios.

==> latexmkrc <==
add_cus_dep( 'tex', 'aux', 0, 'makeexternaldocument' );

sub makeexternaldocument {
    # if the dependency isn't one of the files that this latexmk run will consider, process it
    # without this test, we would get an infinite loop!
    if (!($root_filename eq $_[0]))
    {   # PLEASE ENABLE ONLY ONE OF THE FOLLOWING
        # DEPENDING ON THE ENGINE YOU'RE USING
    
        # FOR PDFLATEX
        system( "latexmk -pdf \"$_[0]\"" );

        # FOR LATEX+DVIPDF
        # system( "latexmk \"$_[0]\"" );

        # FOR XELATEX
        # system( "latexmk -xelatex \"$_[0]\"" );
        
        # FOR LUALATEX
        # system( "latexmk -lualatex \"$_[0]\"" );
   }
}

==> neurips/5_experiments_arxiv.tex <==
% !TeX root = main.tex
\section{Experiments}

\label{sec:experiments}
%We demonstrate the virtue of including Gaussian process priors into interacting systems in a large number of scenarios that differ in function complexity, signal-to-noise ratio and observability of the system.
\edit{
We compare our approach against state-of-the-art methods in a large number of scenarios that differ in function complexity, signal-to-noise ratio and observability of the system.
Our empirical findings suggest that our model leads to improved reliability of long-term predictions while being able to successfully encapsulate autonomous dynamics from interactions effects. 
}
In all our experiments, we use the RK4 ODE solver and ACA library \citep{zhuang20adaptive} for integration and gradient computation.
Due to the space limit, we refer to the Supplementary Material for more detailed information about the experimental setup and comparison methods (see also Table~\ref{tab:references} for an overview). 
We will provide accompanying code based on PyTorch \citep{paszke19pytorch} on GitHub after publication.

\subsection{Experiment Details}
\label{sec:exp-details}
\paragraph{Datasets}
We illustrate the performance of our model on two benchmark datasets: \emph{bouncing balls} \citep{sutskever09recurrent} and \emph{charges} \citep{kipf2018neural}. 
These datasets involve freely moving $\Na=3$ balls that collide with each other 
and $\Na=5$ particles that carry randomly assigned positive or negative charges leading to attraction or repulsion, respectively. 
All simulations are performed in frictionless, square boxes in $2D$. 
We generate $100$ bouncing balls training sequences with different levels of Gaussian perturbations to simulate measurement noise (see Supplementary Section~\ref{sec:supp-data} for noise levels and other details). 
Since the charges dataset requires inferring the charge information, we use $10$k train sequences without observation noise as in \cite{kipf2018neural} and similarly use $500$ training sequences when velocity information is missing.

\paragraph{Partial observability} Prior works typically evaluate their methods on datasets in which the observations consist of position and velocity \citep{battaglia2016interaction, kipf2018neural}. 
However, having access to the full state of an object is for many real-world problems unrealistic,~e.g. 
many tracking devices can measure positions, but cannot measure velocity or acceleration.
%many tracking devices cannot estimate the velocity and acceleration of dynamic objects. 
To test the model performance in such scenarios, we consider an additional bouncing balls dataset in which the velocities are missing. 
On the charges dataset, we assume that position and velocity are observed, but treat the charge information as missing.
%\cagatay{We also learn the charges dataset with the charge information given as input as well as without...}

\newpage
\paragraph{Reported metrics} 
We quantify the model fit by computing the expected log-likelihood (\textsc{ell}) of the data points under the predictive distribution.
Further, we report the mean squared error (\textsc{mse}) between ground truth and predictions over all predicted time steps and over all objects (see Supplementary Section~\ref{sec:supp-data} for the exact definitions).
Each experiment is repeated five times and we report the mean and standard deviation of both metrics on test sequences.

\subsection{Empirical Findings}
\label{sec:exp-findings}
Due to our latent variable construction, ODE state dimensionality $D$ could be arbitrary even though the observations are four-dimensional. 
To choose an appropriate state dimensionality, we study if the model performance can be improved by augmenting the state space with auxiliary dimensions ($D>4$).
Table~\ref{tab:supp:lnode} shows that increasing the model flexibility beyond need leads to overfitting as we observe lower training but significantly higher test error.
Consequently, if not stated otherwise, we use a four-dimensional latent space for each object that corresponds to position and velocity in $x$ and $y$ coordinates and observations consist of their noisy versions.
Next, we discuss the main findings of this study.


\subsubsection{Interacting dynamics are superior over standard formulation}

\begin{wraptable}{r}{8cm}
\vspace{-.65cm}
\centering
	\caption{Comparison of standard and interacting GP-ODE systems on bouncing ball datasets.}
	\label{tab:gps}
	\vspace{.2cm}
    \begin{tabular}{ c | l | r r }
		\toprule
		\textsc{Noise} &
        \multirow{2}{*}{ \textsc{Model} } &
        \multirow{2}{*}{ \textsc{MSE}~$\downarrow$} & 
        \multirow{2}{*}{ \textsc{ELL}~$\uparrow$}  \tabularnewline
        \textsc{Level} & & &  \tabularnewline
        \midrule
        
    \multirow{2}{*}{ \shortstack[c]{ \textsc{No}\\ \textsc{Noise}}}  
    & \textsc{I-GPODE}	 & $\bf{17.3 \pm 1.2}$	 & $\bf{-25.9 \pm 3.6}$ \tabularnewline
	 & \textsc{GPODE}	 & $23.9 \pm 0.9$	 & $-597.6 \pm 28.5$ \tabularnewline
	
	\midrule
	
    \multirow{2}{*}{ \shortstack[c]{ \textsc{Low}\\ \textsc{noise}}} 
    & \textsc{I-GPODE}	 & $\bf{17.8 \pm 0.9}$	 & $\bf{-26.5 \pm 4.5}$ \tabularnewline
	 & \textsc{GPODE}	 & $23.6 \pm 0.7$	 & $-580.8 \pm 19.8$ \tabularnewline
	
	\midrule
	
    \multirow{2}{*}{ \shortstack[c]{ \textsc{High}\\ \textsc{noise}}}  
    & \textsc{I-GPODE}	 & $\bf{18.4 \pm 0.9}$	 & $\bf{-29.4 \pm 1.1}$ \tabularnewline
	 & \textsc{GPODE}	 & $24.5 \pm 1.0$	 & $-569.3 \pm 27.5$ \tabularnewline
	\bottomrule

	\end{tabular}
	% \vspace{-.35cm}
\end{wraptable}

% \paragraph{Interacting dynamics are superior over standard formulation}
We consider three \textit{bouncing ball} datasets with varying noise levels to reflect different levels of problem difficulties.
To demonstrate the merits of our decomposed formulation in Eq.~\eqref{eq:int-ode}, we compare it against a standard, GP-based non-interacting dynamical model (GPODE) in which the time differential takes the whole state vector $\H(t)$ as input \citep{hegde2021bayesian}.
As shown in Table~\ref{tab:gps}, our interaction model consistently outperforms its standard counterpart irrespective of the noise level and function approximator. 
We also note that the results are consistent when we replace the GP approximation with deterministic and Bayesian neural networks (NNs), which indicates the robustness of the inductive bias. (also see Table~\ref{tab:supp:bb3}).
	
\subsubsection{GP approximation yields more calibrated uncertainties}

\begin{wraptable}{r}{8cm}
\vspace{-.65cm}
\centering
	\caption{Comparison of our GP approximation against alternative function approximators.}
	\label{tab:interactions}
	\vspace{.2cm}
	\begin{tabular}{ c | l | r r }
		\toprule
		\textsc{Noise} &
        \multirow{2}{*}{ \textsc{Model} } &
        \multirow{2}{*}{ \textsc{MSE}~$\downarrow$} & 
        \multirow{2}{*}{ \textsc{ELL}~$\uparrow$}  \tabularnewline
        \textsc{Level} & & &  \tabularnewline
        \midrule
        
    \multirow{3}{*}{ \shortstack[c]{ \textsc{No}\\ \textsc{Noise}}}  
    & \textsc{I-GPODE}	 & $17.3 \pm 1.2$	 & $\bf{-25.9 \pm 3.6}$ \tabularnewline
	 & \textsc{I-NODE}	 & $\bf{8.5 \pm 0.9}$	 & $-61.9 \pm 8.6$ \tabularnewline
	 & \textsc{I-BNODE}	 & $20.4 \pm 0.6$	 & $-37.8 \pm 4.2$ \tabularnewline
	
	\midrule
	
    \multirow{3}{*}{ \shortstack[c]{ \textsc{Low}\\ \textsc{noise}}} 
    & \textsc{I-GPODE}	 & $17.8 \pm 0.9$	 & $\bf{-26.5 \pm 4.5}$ \tabularnewline
	 & \textsc{I-NODE}	 & $\bf{13.3 \pm 0.9}$	 & $-96.2 \pm 12.5$ \tabularnewline
	 & \textsc{I-BNODE}	 & $21.0 \pm 0.8$	 & $-36.4 \pm 2.8$ \tabularnewline
	 
	\midrule
	
    \multirow{3}{*}{ \shortstack[c]{ \textsc{High}\\ \textsc{noise}}}  
    & \textsc{I-GPODE}	 & $18.4 \pm 0.9$	 & $\bf{-29.4 \pm 1.1}$ \tabularnewline
	 & \textsc{I-NODE}	 & $\bf{15.6 \pm 1.5}$	 & $-128.9 \pm 23.2$ \tabularnewline
	 & \textsc{I-BNODE}	 & $20.8 \pm 0.7$	 & $-47.6 \pm 10.5$ \tabularnewline
	 
	\bottomrule

	\end{tabular}
	% \vspace{-.35cm}
\end{wraptable}

% \paragraph{GP approximation yields more calibrated uncertainties}
Next, we compare our GP interaction model (I-GPODE) against neural network variants with/without uncertainty (I-NODE, I-BNODE), obtained by replacing GPs with NNs and Bayesian NNs.
The findings in Table~\ref{tab:interactions} strongly indicate that I-GPODE learns better calibrated uncertainties, measured by \textsc{ell}, than I-BNODE and I-NODE (see Figure~\ref{fig:gp-nn-bb} and \ref{fig:supp:gp-nn-bb} for visual illustrations).
In terms of \textsc{mse}, we observe that I-NODE tends to attain the smallest values.
However, increasing noise levels deteriorates the performance of I-NODE and eventually the results become comparable to I-GPODE. 
The results stay consistent when we repeat the experiment with two balls (see Table~\ref{tab:supp:bb2}).

% In sum, these results suggest that \textit{(i)} the proposed interaction framework outperforms standard approaches, \textit{(ii)} our GP approximation is crucial for long-term calibration, and \textit{(iii)} continuous-time systems defined in sufficiently large dimensional spaces lead to superior predictive performance. 

% \paragraph{GP approximation facilitates learning disentangled functions} 

\newpage
\begin{wrapfigure}{r}{8cm}
\vspace{-.65cm}
    \centering
    \includegraphics[width=\linewidth]{gp-nn-transfer-0-5.png} 
    \vspace*{-.75cm}
    \caption{Disentanglement between independent kinematics and interactions. Our model variants are trained on a bouncing ball dataset with three balls and tested with a single ball using the independent dynamics function $\fs$ only. Shown are the mean predictions with circles darkened as time lapses.}
    % We train I-GPODE (ours) and I-NODE on a bouncing ball dataset with three balls, and then predict on a test sequences with a single ball using the independent dynamics function $\fs$ only. Shown are the mean predictions with circles darkened as time lapses.}
    \label{fig:disent}
	\vspace{-.35cm}
\end{wrapfigure}


\subsubsection{GP approximation enables disentangled function learning} 
% \cagatay{Include the study in the rebuttal?}
In the following, we study whether the estimated functions can disentangle independent kinematics from interaction effects.
We train I-GPODE, I-NODE and I-BNODE on a dataset with three balls and evaluate the trained independent dynamics function $\fs$ on a test dataset with one ball (since the test dataset incorporates a single object, the dynamics do not involve the interaction function $\fb$). 
Three test sequences as well as the independent dynamics function predictions are illustrated in Figure~\ref{fig:disent} (see Table~\ref{tab:supp:disent} for a quantitative comparison and Figure~\ref{fig:supp:disent} for additional illustrations).
We observe that I-NODE predictions tend to deviate from the test trajectory more quickly compared to I-GPODE predictions. 
We conjecture that this behaviour is because neural networks are overflexible and thus the learned functions may not necessarily decompose independent kinematics from interaction effects whereas the function-level regularization of I-GPODE helps with disentanglement. 


\begin{wraptable}{r}{8cm}
    \vspace{-.65cm}
    \centering
	\caption{Comparison of I-GPODE variants on a bouncing ball dataset without velocity observations. The suffices ``-L'' and ``-S'' stand for latent variable model and structured state space.
}
	\label{tab:missing-vel}
	\vspace{.2cm}
    \begin{tabular}{l | l | r r }
		\toprule
        \textsc{Noise} & \textsc{Model} & \textsc{MSE}~$\downarrow$ & \textsc{ELL}~$\uparrow$ \tabularnewline
        \midrule
        \multirow{3}{*}{ \shortstack[c]{ \textsc{No}\\ \textsc{noise}}}  
        & \footnotesize{\textsc{I-GPODE}}	 & $24.1 \pm 1.2$	 & $-300 \pm 23$ \tabularnewline
	    & \footnotesize{\textsc{I-GPODE-L}}	 & $23.3 \pm 0.8$	 & $-176 \pm 301$ \tabularnewline
	    & \footnotesize{\textsc{I-GPODE-L-S}} & $\bf{18.2 \pm 1.0}$	 & $\bf{-33 \pm 2}$ \tabularnewline
    	\midrule
    	\midrule
    	\multirow{3}{*}{ \shortstack[c]{ \textsc{Low}\\ \textsc{noise}}}  
        & \footnotesize{\textsc{I-GPODE}}	& $23.3 \pm 0.8$	 & $-239 \pm 11$ \tabularnewline
	    & \footnotesize{\textsc{I-GPODE-L}}	  & $47.0 \pm 47.4$	 & $-761 \pm 922$ \tabularnewline
	    & \footnotesize{\textsc{I-GPODE-L-S}} & $\bf{20.5 \pm 0.9}$	 & $\bf{-76 \pm 22}$ \tabularnewline
    	\midrule
    	\midrule
    	\multirow{3}{*}{ \shortstack[c]{ \textsc{High}\\ \textsc{noise}}}  
        & \footnotesize{\textsc{I-GPODE}}	 & $23.8 \pm 0.7$	 & $-254 \pm 16$ \tabularnewline
	    & \footnotesize{\textsc{I-GPODE-L}}	 & $119.3 \pm 94.3$	 & $-920 \pm 982$ \tabularnewline
	    & \footnotesize{\textsc{I-GPODE-L-S}}  & $\bf{21.8 \pm 0.7}$	 & $\bf{-115 \pm 19}$ \tabularnewline
    	\bottomrule
	\end{tabular}
	\vspace{-.35cm}
\end{wraptable}

% \paragraph{Structured dynamics improve latent dynamics learning} 
\subsubsection{Structured dynamics improve latent dynamics learning} 
In our last bouncing ball experiment, we move to a setting in which the velocities are no longer observed.
First, we keep the velocities as latent states and contrast two variants of our model, i.e. with structured latent space  (I-GPODE-L-S) and with unstructured latent space (I-GPODE-L).
As shown in Table~\ref{tab:missing-vel}, injecting strong prior knowledge helps
in this challenging setting in which the first order model
clearly fails (see also Table~\ref{tab:supp:missing-vel} for training results).
%As expected, the difference between these two approaches become insignificant in the easier, fully observed setting; hence, the results are omitted.
Finally, we compare I-GPODE-L-S with I-GPODE, which drops the velocity component from the latent space (hence learning the dynamics in the data space).
%contrast two variants of our model, i.e., with and without latent variables, on a partially observed bouncing ball dataset. 
As demonstrated in Table~\ref{tab:missing-vel}, I-GPODE is clearly outperformed by I-GPODE-L-S. 
It can thus be suggested that our latent variable construction is necessary in presence of missing states.
% Since the unknown true dynamics involve second-order velocity information, 
% As shown in \cite{dupont2019augmented}, data-space ODEs fail to learn such intersecting sequences, which in our case led to numerical errors during training the vanilla GP-ODE baseline.
% When the velocity information is omitted, the remaining data trajectories (positions) occasionally intersect (see figure \cagatay{appendix figure}).

%\paragraph{Latent dynamical systems} 
%Second, we check whether latent modeling has any potential drawbacks.
%For this purpose, we compare standard NODE \citep{chen2018neural} against its latent counterpart NODE-L \citep{rubanova19latent} in fully observed setups.
% which are constructed by augmenting the state space with auxiliary dimensions,  
%As shown in Table~\ref{tab:supp:lnode}, NODE-L leads to significantly higher test error across all noise levels and hence is not included in our main comparisons. 


%The underlying physical system can be inferred by the auto-regressive function $\f_s$ in presence of a single ball, while the multiple ball scenarios require learning the interaction function $\f_b$ as well. 
% Since we have full control over data simulation, we consider a variety of simulations to highlight different aspects of our model. 

% \paragraph{Baseline models} The first two baselines considered are the vanilla NODE model \citep{chen2018neural} and latent NODE (LNODE) \citep{rubanova19latent}. These comparisons aim to illustrate the shortcomings of data-space modeling and that our latent variable construction \eqref{eq:lv} can match the level of accuracy achieved by a much more powerful and complex latent model without sacrificing interpretability. To demonstrate the merits of our probabilistic dynamics, we compare our method against \emph{iNODE} and \emph{idNODE}, where our GP approximations are replaced with vanilla and dropout neural networks.


\begin{wraptable}{r}{8cm}
    \vspace{-.65cm}
    \centering
	\caption{Comparison of interacting GPODE and NODE systems on the charges dataset (no noise).}
	\label{tab:charges}
	\vspace{.2cm}
    \begin{tabular}{l | l r r }
		\toprule
        & \textsc{Model} & \textsc{MSE}~$\downarrow$ & \textsc{ELL}~$\uparrow$ \tabularnewline
        \midrule 
    	\multirow{2}{*}{ \shortstack[c]{ \footnotesize{\textsc{Without}}\\
    	\footnotesize{\textsc{Global}}\\
    	\footnotesize{\textsc{Latents}}}}  
    	& \small{\textsc{I-GPODE}} & $19.2 \pm 0.9$	 & $-171 \pm 7$ \tabularnewline
    	& \vspace*{.05cm} \small{\textsc{I-NODE}}	 & $14.1 \pm 0.8$	 & $-460 \pm 36$ \tabularnewline
        \midrule
        \midrule
    	\multirow{4}{*}{\vspace*{-.2cm} \shortstack[c]{ 
    	\footnotesize{\textsc{With}}\\
    	\footnotesize{\textsc{Global}}\\
    	\footnotesize{\textsc{Latents}}}} 
    	& \small{\textsc{I-GPODE}} & $15.4 \pm 2.3$	 & $-172 \pm 88$ \tabularnewline
    	& \small{\textsc{I-NODE}}	 & $9.9 \pm 0.6$	 & $-282 \pm 14$ \tabularnewline
        \cmidrule{2-4}
    	& \small{\textsc{I-GPODE-S}} & $12.9 \pm 2.1$	 & $\mathbf{-177 \pm 60}$ \tabularnewline
    	& \small{\textsc{I-NODE-S}}	 & $\mathbf{9.7 \pm 0.2}$	 & $-282 \pm 8$ \tabularnewline
        \midrule
        \midrule
    	\multirow{2}{*}{\vspace*{-.2cm} \shortstack[c]{ 
    	\footnotesize{\textsc{Globals}}\\
    	\footnotesize{\textsc{Observed}}}}  
    	& \small{\textsc{I-GPODE}} & $10.7 \pm 1.1$	 & $-97 \pm 9$ \tabularnewline
    	& \small{\textsc{I-NODE}}	 & $7.5 \pm 1.2$	 & $-148 \pm 27$ \tabularnewline
	\bottomrule
	\end{tabular}
	\vspace{-.35cm}
\end{wraptable}


\subsubsection{Global latent variables boost performance}
% \paragraph{Global latent variables boost performance}
In the final part of the experiments, we consider a more challenging dataset of charged particles. Since the dynamics are modulated by unknown charges, we turn to our global latent variable formulation. In other words, our learning task becomes simultaneously inferring the functions $\fs$ and $\fb$, the initial latent states $\H_1$, as well as a latent variable $\bc^a \in \R$ associated with each observed trajectory $\y_{1:N}^a$. To form the upper and lower performance bounds, we include two baselines in which the charges are either observed or completely dropped from the model description.% (see Table~\ref{tab:charges}).
The results are shown in Table~\ref{tab:charges}. 
%To gain a better understanding of the findings, we include two baselines: charges are observed and charges are dropped from the model which form the upper and lower performance bounds.
%As expected, the results improve with global latent variables included. 
\edit{
We notice that the structured state space formulation boosts the performance of I-GPODE.
However, the effect is less pronounced compared to the previous setting in which dynamic information is missing.
}
%We notice that the structured state space formulation significantly outperforms the standard I-GPODE model. %boosts the performance of I-GPODE.
%We conjencture that restraining the latent space helps in separating dynamic effects from static ones, leading to this performance boost.
%performance closer to the setting with observed charges. 
See Table~\ref{tab:supp:charges} for more results with different global variable encoders.

==> neurips/5experiments.tex <==
% !TeX root = main.tex

\begin{figure}
    \centering
    \includegraphics[width=.75\linewidth]{gp-nn-transfer-0-5.png} 
    \vspace*{-.5cm}
    \caption{
    {Disentanglement between independent kinematics and interaction components.}
    We train I-GPODE (ours) and I-NODE on a bouncing ball dataset with three balls, and then predict on a test sequences with a single ball using the independent dynamics function $\fs$ only. Shown are the mean predictions with the circles darkened as time lapses.
    %Mean predictions of the independent dynamics function $\fs$ of GPODE (ours) and NODE trained on a bouncing ball dataset with three balls. The circles are darkened over time.
    % \cagatay{Make an experiment with smaller $\beta$ in front of KL to check the GP initial value and slow vector field problems.}
    }
    \label{fig:disent}
\end{figure}


\section{Experiments}

\label{sec:experiments}
We demonstrate the virtue of including Gaussian Process priors into interacting systems in a large number of scenarios that differ in function complexity, signal-to-noise ratio and observability of the system.
In all our experiments, we use the RK4 ODE solver and ACA library \citep{zhuang20adaptive} for integration and gradient computation.
Due to the space limit, we refer to the Supplementary Material for more detailed information about the experimental setup and comparison methods (see also Table~\ref{tab:references} for an overview). 
We will provide accompanying code based on PyTorch \citep{paszke19pytorch} on GitHub after publication.

\subsection{Experiment Details}
\label{sec:exp-details}
\paragraph{Datasets}
We illustrate the performance of our model on two benchmark datasets: \emph{bouncing balls} \citep{sutskever09recurrent} and \emph{charges} \citep{kipf2018neural}. 
These datasets involve freely moving $\Na=3$ balls that collide with each other 
and $\Na=5$ particles that carry randomly assigned positive or negative charges leading to attraction or repulsion, respectively. 
All simulations are performed in frictionless, square boxes in $2D$. 
We generate $100$ bouncing balls training sequences with different levels of Gaussian perturbations to simulate measurement noise (see Supplementary Section~\ref{sec:supp-data} for details). Since the charges dataset requires inferring the charge information, we use $10$k train sequences without observation noise as in \cite{kipf2018neural} and similarly use $500$ training sequences when velocity information is missing.

\paragraph{Partial observability} Prior works typically evaluate their methods on datasets in which the observations consist of position and velocity \citep{battaglia2016interaction, kipf2018neural}. 
However, having access to the full state of an object is for many real-world problems unrealistic,~e.g. 
many tracking devices can measure positions, but cannot measure velocity or acceleration.
%many tracking devices cannot estimate the velocity and acceleration of dynamic objects. 
To test the model performance in such scenarios, we consider an additional bouncing balls dataset in which the velocities are missing. 
On the charges dataset, we assume that position and velocity are given, but treat the charge information as missing.
%\cagatay{We also learn the charges dataset with the charge information given as input as well as without...}

\paragraph{Reported metrics} 
We quantify the model fit by computing the expected log-likelihood (\textsc{ell}) of the data points under the predictive distribution.
Further, we report the mean squared error (\textsc{mse}) between ground truth and predictions over all predicted time steps and over all objects (see Supplementary Section~\ref{sec:supp-data} for the exact definitions).
Each experiment is repeated five times and we report the mean and standard deviation of both metrics on test sequences.


\subsection{Empirical Findings}
\label{sec:exp-findings}
\paragraph{Auxillary ODE states deteriorate model performance}
Due to our latent variable construction, ODE state dimensionality $D$ could be arbitrary even though the observations are four-dimensional. 
To choose the appropriate state dimensionality, we first study if the model performance can be improved by augmenting the state space with auxiliary dimensions ($D>4$).
Our results in Table~\ref{tab:supp:lnode} indicate that increasing the model flexibility beyond need leads to overfitting as we observe low training error, but significantly higher test error.
Consequently, if not stated otherwise, we use a four-dimensional latent space for each object that corresponds to position and velocity in $x$ and $y$ coordinates and the observations consists of their noisy versions.


\paragraph{Interacting dynamics are superior over standard formulation}
We consider three \textit{bouncing ball} datasets with varying noise levels to reflect different levels of problem difficulties.
To demonstrate the merits of our decomposed formulation in eq.~\eqref{eq:int-ode}, we compare it against a standard, GP-based non-interacting dynamical model (GPODE) in which the time differential takes the whole state vector $\H(t)$ as input \citep{hegde2021bayesian}.
As shown in Table~\ref{tab:gps}, our interaction model consistently outperforms its standard counterpart irrespective of the noise level and function approximator. 
We also note that the results are consistent when we replace the GP approximation with deterministic and Bayesian neural networks (NNs), which indicates the robustness of the inductive bias. (see Table~\ref{tab:supp:bb3}).
	
\input{table21}
\input{table22}


\paragraph{GP approximation yields more calibrated uncertainties}
Next, we compare our GP interaction (I-GPODE) formulation with neural network variants with and without uncertainty (I-NODE, I-BNODE), which are obtained by replacing GPs with NNs and Bayesian NNs.
The findings in Table~\ref{tab:interactions} strongly indicate that I-GPODE learns better calibrated uncertainties, as measured by \textsc{ell}, than I-BNODE and I-NODE (see Figure~\ref{fig:gp-nn-bb} and \ref{fig:supp:gp-nn-bb} for visual illustrations).
In terms of \textsc{mse}, we observe that I-NODE tends to attain the smallest values.
However, increasing noise levels leads to a deteriorated performance of I-NODE and eventually the results become comparable to I-GPODE. 
The results stay consistent when we repeat the experiment with two balls (see Table~\ref{tab:supp:bb2}).

% In sum, these results suggest that \textit{(i)} the proposed interaction framework outperforms standard approaches, \textit{(ii)} our GP approximation is crucial for long-term calibration, and \textit{(iii)} continuous-time systems defined in sufficiently large dimensional spaces lead to superior predictive performance. 

\paragraph{GP approximation facilitates learning disentangled functions} 
\cagatay{Include the study in the rebuttal}
In the following, we study whether the estimated functions can disentangle independent kinematics from interaction effects.
We train I-GPODE, I-NODE and I-BNODE on a dataset with three balls and evaluate the trained independent dynamics function $\fs$ on a test dataset with one ball (since the test dataset incorporates a single object, the dynamics do not involve the interaction function $\fb$). 
Three test sequences as well as the independent dynamics function predictions are illustrated in Figure~\ref{fig:disent} (see Table~\ref{tab:supp:disent} for a quantitative comparison and Figure~\ref{fig:supp:disent} for additional illustrations).
We observe that I-NODE predictions tend to deviate from the test trajectory more quickly compared to I-GPODE predictions. 
We conjecture that this behaviour is because neural networks are overflexible and thus the learned functions may not necessarily decompose independent kinematics from interaction effects whereas the function-level regularization of I-GPODE helps with disentanglement. 

\paragraph{Structured dynamics improve latent dynamics learning} 
In our last bouncing ball experiment, we move to a setting in which the velocities are no longer observed.
First, we keep the velocities as latent states and contrast two variants of our model, i.e. with structured latent space  (I-GPODE-L-S) and with unstructured latent space (I-GPODE-L).
As shown in Table~\ref{tab:missing-vel}, injecting strong prior knowledge helps
in this challenging setting in which the first order model
clearly fails (see also Table~\ref{tab:supp:missing-vel} for training results).
%As expected, the difference between these two approaches become insignificant in the easier, fully observed setting; hence, the results are omitted.
Finally, we compare I-GPODE-L-S with I-GPODE, which drops the velocity component from the latent space.
%contrast two variants of our model, i.e., with and without latent variables, on a partially observed bouncing ball dataset. 
As demonstrated in Table~\ref{tab:missing-vel}, I-GPODE is unable to learn the dynamics and outperformed by I-GPODE-L-S. 
It can thus be suggested that our latent variable construction is necessary in presence of missing states.
% Since the unknown true dynamics involve second-order velocity information, 
% As shown in \cite{dupont2019augmented}, data-space ODEs fail to learn such intersecting sequences, which in our case led to numerical errors during training the vanilla GP-ODE baseline.
% When the velocity information is omitted, the remaining data trajectories (positions) occasionally intersect (see figure \cagatay{appendix figure}).

%\paragraph{Latent dynamical systems} 
%Second, we check whether latent modeling has any potential drawbacks.
%For this purpose, we compare standard NODE \citep{chen2018neural} against its latent counterpart NODE-L \citep{rubanova19latent} in fully observed setups.
% which are constructed by augmenting the state space with auxiliary dimensions,  
%As shown in Table~\ref{tab:supp:lnode}, NODE-L leads to significantly higher test error across all noise levels and hence is not included in our main comparisons. 


%The underlying physical system can be inferred by the auto-regressive function $\f_s$ in presence of a single ball, while the multiple ball scenarios require learning the interaction function $\f_b$ as well. 
% Since we have full control over data simulation, we consider a variety of simulations to highlight different aspects of our model. 

% \paragraph{Baseline models} The first two baselines considered are the vanilla NODE model \citep{chen2018neural} and latent NODE (LNODE) \citep{rubanova19latent}. These comparisons aim to illustrate the shortcomings of data-space modeling and that our latent variable construction \eqref{eq:lv} can match the level of accuracy achieved by a much more powerful and complex latent model without sacrificing interpretability. To demonstrate the merits of our probabilistic dynamics, we compare our method against \emph{iNODE} and \emph{idNODE}, where our GP approximations are replaced with vanilla and dropout neural networks.



% \begin{table*}
%     \begin{center}
% 	\caption{Experiments Outline}
% 	\label{tab:exps}
% 	\begin{tabular}{llllp{6cm}}
% 		\toprule
% 		\textsc{Experiment} & \textsc{Obs} &\textsc{Latent} & \textsc{Methods} & \textsc{Goal} \tabularnewline
% 		\midrule
% 		BB: 2 $\rightarrow$ 1,2,3 & Pos, vel & - & GP-SA, NN-SA, GP-MA, NN-MA &
% 	Interaction function helps \newline Calibration requires function uncertainty.
% 		\tabularnewline
% 	BB: 2 $\rightarrow$ 1,2,3 & Pos & vel  &  All methods &
% 		Interaction function helps,\newline Latent dims/space needed, \newline Calibration requires function uncertainty. \tabularnewline
% 		BB: $2 \rightarrow 1$ & Pos,vel && 
% 		GP-MA, NN-MA, (B)NN-MA & GP-based dynamics are indeed disentangled.  \tabularnewline
% 		BB: 2 & Pos & Vel & GP-MA-L, GP-MA-L(2nd order) &  Second-order dynamics help  \tabularnewline 
% 		Spring & Pos & Inter & All methods &
% 		Interaction function helps \newline Latent dims/space needed \newline Calibration requires function uncertainty. \tabularnewline
% 	Charging Particles & Pos & Property & All methods &
% 		Interaction function helps \newline Latent dims/space needed \newline Calibration requires function uncertainty. \tabularnewline
% 		\bottomrule
% 	\end{tabular}
%     \end{center}
% \end{table*}

\paragraph{Global latent variables boost performance}
In the final part of the experiments, we consider a more challenging dataset of charged particles. Since the dynamics are modulated by unknown charges, we turn to our global latent variable formulation. In other words, our learning task becomes simultaneously inferring the functions $\fs$ and $\fb$, the initial latent states $\H_1$, as well as a latent variable $\bc^a \in \R$ associated with each observed trajectory $\y_{1:N}^a$. To form the upper and lower performance bounds, we include two baselines in which the charges are either observed or completely dropped from the model description.% (see Table~\ref{tab:charges}).
The results are shown in Table~\ref{tab:charges}. 
%To gain a better understanding of the findings, we include two baselines: charges are observed and charges are dropped from the model which form the upper and lower performance bounds.
%As expected, the results improve with global latent variables included. 
We notice that the structured state space formulation %significantly outperforms the standard I-GPODE model. 
boosts the performance of I-GPODE.
\edit{However, the effect is less pronounced compared to the previous setting in which dynamic information is missing.
}
%We conjencture that restraining the latent space helps in separating dynamic effects from static ones, leading to this performance boost.
%performance closer to the setting with observed charges. 
See Table~\ref{tab:supp:charges} for more results with different global variable encoders.

\input{table3}

==> neurips/7checklist.tex <==

\section*{Checklist}
\begin{enumerate}


\item For all authors...
\begin{enumerate}
  \item Do the main claims made in the abstract and introduction accurately reflect the paper's contributions and scope?
    \answerYes{}
  \item Did you describe the limitations of your work?
    \answerYes{}
  \item Did you discuss any potential negative societal impacts of your work?
    \answerYes{}
  \item Have you read the ethics review guidelines and ensured that your paper conforms to them?
    \answerYes{}
\end{enumerate}


\item If you are including theoretical results...
\begin{enumerate}
  \item Did you state the full set of assumptions of all theoretical results?
    \answerNA{}
        \item Did you include complete proofs of all theoretical results?
    \answerNA{}
\end{enumerate}


\item If you ran experiments...
\begin{enumerate}
  \item Did you include the code, data, and instructions needed to reproduce the main experimental results (either in the supplemental material or as a URL)?
    \answerYes{See supplements Sec.~\ref{sec:supp-data} and the attached code}
  \item Did you specify all the training details (e.g., data splits, hyperparameters, how they were chosen)?
    \answerYes{See the ``Dynamics approximations and hyper-parameter selection'' paragraph in the supplements}
    \item Did you report error bars (e.g., with respect to the random seed after running experiments multiple times)?
    \answerYes{}
    \item Did you include the total amount of compute and the type of resources used (e.g., type of GPUs, internal cluster, or cloud provider)?
    \answerYes{See the ``Training details'' paragraph in the supplements}
\end{enumerate}


\item If you are using existing assets (e.g., code, data, models) or curating/releasing new assets...
\begin{enumerate}
  \item If your work uses existing assets, did you cite the creators?
    \answerYes{See Sec.~\ref{sec:exp-details}}
  \item Did you mention the license of the assets?
    \answerYes{}
  \item Did you include any new assets either in the supplemental material or as a URL?
    \answerYes{Our source code is attached}
  \item Did you discuss whether and how consent was obtained from people whose data you're using/curating?
    \answerNo{}
  \item Did you discuss whether the data you are using/curating contains personally identifiable information or offensive content?
    \answerNA{}
\end{enumerate}


\item If you used crowdsourcing or conducted research with human subjects...
\begin{enumerate}
  \item Did you include the full text of instructions given to participants and screenshots, if applicable?
    \answerNA{}
  \item Did you describe any potential participant risks, with links to Institutional Review Board (IRB) approvals, if applicable?
    \answerNA{}
  \item Did you include the estimated hourly wage paid to participants and the total amount spent on participant compensation?
    \answerNA{}
\end{enumerate}


\end{enumerate}


==> table2.tex <==

\begin{table}
\centering
	\caption{Comparison on fully observed bouncing ball dataset.
	Each row group corresponds to a different noise level (no, low, high).
	See Table~\ref{tab:references} for more details on the comparison methods.}
	% less ../exp_logs/gpsa\[1-30\].2420764.1.err)
	% results are in nn-gp-sa-ma_balls-3_order-1_obsvel-1
	\label{tab:main-comp}
	\vspace{.2cm}
    \begin{tabular}{ c | l | r r }
		\toprule
		\textsc{Noise} &
        \multirow{2}{*}{ \textsc{Model} } &
        \multirow{2}{*}{ \textsc{MSE}~$\downarrow$} & 
        \multirow{2}{*}{ \textsc{ELL}~$\uparrow$}  \tabularnewline
        \textsc{Level} & & &  \tabularnewline
        \midrule
        
    \multirow{6}{*}{ \shortstack[c]{ \textsc{No}\\ \textsc{Noise}}}  
    & \textsc{I-GPODE}	 & $17.29 \pm 1.18$	 & $\bf{-25.88 \pm 3.56}$ \tabularnewline
	 & \textsc{I-NODE}	 & $\bf{8.45 \pm 0.93}$	 & $-61.90 \pm 8.63$ \tabularnewline
	 & \textsc{I-BNODE}	 & $20.39 \pm 0.62$	 & $-37.81 \pm 4.23$ \tabularnewline
	\cmidrule{2-4}
	 & \textsc{GPODE}	 & $23.89 \pm 0.91$	 & $-597.63 \pm 28.48$ \tabularnewline
	 & \textsc{NODE}     & $30.07 \pm 1.63$	 & $-911.95 \pm 50.17$ \tabularnewline
	 & \textsc{BNODE}	 & $23.22 \pm 0.60$	 & $-56.57 \pm 9.41$ \tabularnewline
	
	\midrule
	\midrule
	
    \multirow{6}{*}{ \shortstack[c]{ \textsc{Low}\\ \textsc{noise}}} 
    & \textsc{I-GPODE}	 & $17.76 \pm 0.89$	 & $\bf{-26.48 \pm 4.54}$ \tabularnewline
	 & \textsc{I-NODE}	 & $\bf{13.33 \pm 0.93}$	 & $-96.15 \pm 12.47$ \tabularnewline
	 & \textsc{I-BNODE}	 & $20.98 \pm 0.78$	 & $-36.40 \pm 2.77$ \tabularnewline
	\cmidrule{2-4}
	 & \textsc{GPODE}	 & $23.63 \pm 0.72$	 & $-580.82 \pm 19.83$ \tabularnewline
	 & \textsc{NODE}	 & $30.84 \pm 1.94$	 & $-757.27 \pm 56.12$ \tabularnewline
	 & \textsc{BNODE}	 & $22.99 \pm 0.77$	 & $-51.98 \pm 5.68$ \tabularnewline
	
	\midrule
	\midrule
	
    \multirow{6}{*}{ \shortstack[c]{ \textsc{High}\\ \textsc{noise}}}  
    & \textsc{I-GPODE}	 & $18.36 \pm 0.86$	 & $\bf{-29.38 \pm 1.14}$ \tabularnewline
	 & \textsc{I-NODE}	 & $\bf{15.60 \pm 1.47}$	 & $-128.89 \pm 23.21$ \tabularnewline
	 & \textsc{I-BNODE}	 & $20.84 \pm 0.72$	 & $-47.63 \pm 10.51$ \tabularnewline
	\cmidrule{2-4}
	 & \textsc{GPODE}	 & $24.25 \pm 1.00$	 & $-569.29 \pm 27.46$ \tabularnewline
	 & \textsc{NODE}	 & $29.86 \pm 1.38$	 & $-567.69 \pm 47.49$ \tabularnewline
	 & \textsc{BNODE}	 & $22.33 \pm 0.52$	 & $-52.49 \pm 7.41$ \tabularnewline
	\bottomrule

	\end{tabular}
	\vspace{-6mm}
\end{table}

==> table21.tex <==

\begin{table}
\centering
	\caption{Comparison of standard and interacting GP-ODE systems on bouncing ball datasets.}
	\label{tab:gps}
	\vspace{.2cm}
    \begin{tabular}{ c | l | r r }
		\toprule
		\textsc{Noise} &
        \multirow{2}{*}{ \textsc{Model} } &
        \multirow{2}{*}{ \textsc{MSE}~$\downarrow$} & 
        \multirow{2}{*}{ \textsc{ELL}~$\uparrow$}  \tabularnewline
        \textsc{Level} & & &  \tabularnewline
        \midrule
        
    \multirow{2}{*}{ \shortstack[c]{ \textsc{No}\\ \textsc{Noise}}}  
    & \textsc{I-GPODE}	 & $\bf{17.29 \pm 1.18}$	 & $\bf{-25.88 \pm 3.56}$ \tabularnewline
	 & \textsc{GPODE}	 & $23.89 \pm 0.91$	 & $-597.63 \pm 28.48$ \tabularnewline
	
	\midrule
	
    \multirow{2}{*}{ \shortstack[c]{ \textsc{Low}\\ \textsc{noise}}} 
    & \textsc{I-GPODE}	 & $\bf{17.76 \pm 0.89}$	 & $\bf{-26.48 \pm 4.54}$ \tabularnewline
	 & \textsc{GPODE}	 & $23.63 \pm 0.72$	 & $-580.82 \pm 19.83$ \tabularnewline
	
	\midrule
	
    \multirow{2}{*}{ \shortstack[c]{ \textsc{High}\\ \textsc{noise}}}  
    & \textsc{I-GPODE}	 & $\bf{18.36 \pm 0.86}$	 & $\bf{-29.38 \pm 1.14}$ \tabularnewline
	 & \textsc{GPODE}	 & $24.25 \pm 1.00$	 & $-569.29 \pm 27.46$ \tabularnewline
	\bottomrule

	\end{tabular}
\end{table}

==> table22.tex <==

\begin{table}
\centering
	\caption{Comparison of our GP approximation against alternative function approximators.}
	\label{tab:interactions}
	\vspace{.2cm}
    \begin{tabular}{ c | l | r r }
		\toprule
		\textsc{Noise} &
        \multirow{2}{*}{ \textsc{Model} } &
        \multirow{2}{*}{ \textsc{MSE}~$\downarrow$} & 
        \multirow{2}{*}{ \textsc{ELL}~$\uparrow$}  \tabularnewline
        \textsc{Level} & & &  \tabularnewline
        \midrule
        
    \multirow{3}{*}{ \shortstack[c]{ \textsc{No}\\ \textsc{Noise}}}  
    & \textsc{I-GPODE}	 & $17.29 \pm 1.18$	 & $\bf{-25.88 \pm 3.56}$ \tabularnewline
	 & \textsc{I-NODE}	 & $\bf{8.45 \pm 0.93}$	 & $-61.90 \pm 8.63$ \tabularnewline
	 & \textsc{I-BNODE}	 & $20.39 \pm 0.62$	 & $-37.81 \pm 4.23$ \tabularnewline
	
	\midrule
	
    \multirow{3}{*}{ \shortstack[c]{ \textsc{Low}\\ \textsc{noise}}} 
    & \textsc{I-GPODE}	 & $17.76 \pm 0.89$	 & $\bf{-26.48 \pm 4.54}$ \tabularnewline
	 & \textsc{I-NODE}	 & $\bf{13.33 \pm 0.93}$	 & $-96.15 \pm 12.47$ \tabularnewline
	 & \textsc{I-BNODE}	 & $20.98 \pm 0.78$	 & $-36.40 \pm 2.77$ \tabularnewline
	 
	\midrule
	
    \multirow{3}{*}{ \shortstack[c]{ \textsc{High}\\ \textsc{noise}}}  
    & \textsc{I-GPODE}	 & $18.36 \pm 0.86$	 & $\bf{-29.38 \pm 1.14}$ \tabularnewline
	 & \textsc{I-NODE}	 & $\bf{15.60 \pm 1.47}$	 & $-128.89 \pm 23.21$ \tabularnewline
	 & \textsc{I-BNODE}	 & $20.84 \pm 0.72$	 & $-47.63 \pm 10.51$ \tabularnewline
	 
	\bottomrule

	\end{tabular}
\end{table}

==> table3.tex <==

\begin{table}[t]
    \centering
	\caption{Comparison of I-GPODE variants on a bouncing ball dataset without velocity observations. Note that the suffix ``-S'' stands for structured state space and each row group corresponds to a different noise level (no, low, high).
%	See Table~\ref{tab:references} for more details on the comparison methods.
}
	\label{tab:missing-vel}
	\vspace{.2cm}
    \begin{tabular}{l r r }
		\toprule
        \textsc{Model} & \textsc{MSE}~$\downarrow$ & \textsc{ELL}~$\uparrow$ \tabularnewline
        \midrule
        \textsc{I-GPODE}	 & $24.11 \pm 1.18$	 & $-300.78 \pm 23.35$ \tabularnewline
	    \textsc{I-GPODE-L}	 & $23.32 \pm 0.76$	 & $-176.04 \pm 30.98$ \tabularnewline
	    \textsc{I-GPODE-L-S} & $\bf{18.22 \pm 1.01}$	 & $\bf{-33.45 \pm 1.96}$ \tabularnewline
    	\midrule
    	\midrule
    	\textsc{I-GPODE}	& $23.26 \pm 0.77$	 & $-239.37 \pm 11.10$ \tabularnewline
	    \textsc{I-GPODE-L}	  & $47.01 \pm 47.38$	 & $-760.60 \pm 921.56$ \tabularnewline
	    \textsc{I-GPODE-L-S} & $\bf{20.46 \pm 0.92}$	 & $\bf{-76.35 \pm 22.48}$ \tabularnewline
    	\midrule
    	\midrule
    	\textsc{I-GPODE}	 & $23.77 \pm 0.68$	 & $-254.34 \pm 16.43$ \tabularnewline
	    \textsc{I-GPODE-L}	 & $119.24 \pm 94.27$	 & $-920.27 \pm 982.10$ \tabularnewline
	    \textsc{I-GPODE-L-S}  & $\bf{21.80 \pm 0.69}$	 & $\bf{-115.50 \pm 19.20}$ \tabularnewline
    	\bottomrule
	\end{tabular}
%	\vspace{-10mm}
%\end{table}
%\begin{table}
  %  \centering
	\caption{Comparison of interacting GPODE and NODE systems on the charges dataset.}
	\label{tab:charges}
	\vspace{.2cm}
    \begin{tabular}{l | l r r }
		\toprule
        & \textsc{Model} & \textsc{MSE}~$\downarrow$ & \textsc{ELL}~$\uparrow$ \tabularnewline
        \midrule
    	\multirow{2}{*}{ \shortstack[c]{ \footnotesize{\textsc{Without}}\\
    	\footnotesize{\textsc{Global}}\\
    	\footnotesize{\textsc{Latents}}}} & \small{\textsc{I-GPODE}} & $19.2 \pm 0.9$	 & $-171 \pm 7$ \tabularnewline
    	& \small{\textsc{I-NODE}}	 & $14.1 \pm 0.8$	 & $-460 \pm 36$ \tabularnewline
        \midrule
        \midrule
    	\multirow{4}{*}{\vspace*{-.2cm} \shortstack[c]{ 
    	\footnotesize{\textsc{With}}\\
    	\footnotesize{\textsc{Global}}\\
    	\footnotesize{\textsc{Latents}}}} 
    	& \small{\textsc{I-GPODE}} & $15.4 \pm 2.3$	 & $-172 \pm 88$ \tabularnewline
    	& \small{\textsc{I-NODE}}	 & $9.9 \pm 0.6$	 & $-282 \pm 14$ \tabularnewline
        \cmidrule{2-4}
    	& \small{\textsc{I-GPODE-S}} & $12.9 \pm 2.1$	 & $-177 \pm 60$ \tabularnewline
    	& \small{\textsc{I-NODE-S}}	 & $9.7 \pm 0.2$	 & $-282 \pm 8$ \tabularnewline
        \midrule
        \midrule
    	\multirow{2}{*}{\vspace*{-.2cm} \shortstack[c]{ 
    	\footnotesize{\textsc{Globals}}\\
    	\footnotesize{\textsc{Observed}}}}  
    	& \small{\textsc{I-GPODE}} & $10.7 \pm 1.1$	 & $-97 \pm 9$ \tabularnewline
    	& \small{\textsc{I-NODE}}	 & $7.5 \pm 1.2$	 & $-148 \pm 27$ \tabularnewline
	\bottomrule
	\end{tabular}
	\vspace{-5mm}
\end{table}
